Can Telematics Improve Driving Style? The Use of Behavioural Data in Motor Insurance

Motor insurance can use telematics data not only to understand the individual driving style, but also to implement innovative coaching strategies that feed back to the drivers, through an app, the aggregated information extracted from the data. The purpose is to encourage an improvement in their driving style. Precondition for this improvement is that drivers are digitally engaged, that is, they interact with the app. Our hypothesis is that the effectiveness of current experimentations depends on the integration of two distinct types of behavioural data: behavioural data on driving style and behavioural data on users' interaction with the app. Based on the empirical investigation of the dataset of a company selling a telematics motor insurance policy, our research shows that there is a correlation between engagement with the app and improvement of driving style, but the analysis must distinguish different groups of users with different driving abilities, and take into account time differences. Our findings contribute to clarify the methodological challenges that must be addressed when exploring engagement and coaching effectiveness in proactive insurance policies. We conclude by discussing the possibility and difficulties of tracking and using second-order behavioural data related to policyholder engagement with the app.

==> EngagAsPrecondition.tex <==
% \section{Engagement (meglio Coaching?) in usage-based-insurance}\label{sec:NewUniqueChapter}


\subsection{Engagement as a precondition for coaching}\label{sec:engag}
% \section{Engagement as a precondition for coaching}\label{sec:engag}

\red{Spostiamo nell'introduction, con un po' di revisione?}

The feedback loop can achieve a coaching effect only in the case policyholders are engaged. As explained in the Introduction, by \textit{engagement} we mean the active dealing of policyholders with the information fed back by the insurance company via the various functionalities of the app \cite{asimakopoulos2017motivation, Bucher2020engaged}. Without such engagement, it is impossible to say whether an improvement in driving behaviour is the result of coaching or simply a matter of chance. For this reason, the usual UBI formulation should be clarified. 
The success of proactive strategies implemented by insurance companies is, in fact, based on two different types of behaviour: not only the driving behaviour of policyholders but also their interaction with the app, i.e., their being engaged. The use of the app is itself a behaviour tracked by telematics apps, as well as driving behaviour. Insurance companies selling PHYD insurance policies collect a lot of data about both behaviours, use of the car, and use of the app. This is, in our opinion, a crucial novelty.
Behavioural data are considered a “remarkable advance” in automobile insurance \cite[p.~662]{guillen2019use}. Previously, the insurance industry could only use variables related to fixed characteristics of the policyholder and the vehicle, many of which, such as age and gender, are not causally related to the risk of getting into a crash. They are proxy variables.
Behavioural variables, instead, are causally related to the risk of road accidents and promise to enable personalised tarification, which may be considered a fairer policy premium setting system \cite{meyers2018enacting, cevoliniesposito2022from}. Moreover, as we have seen, behavioural data processing can be carried out to implement coaching strategies and possibly improve policyholders’ driving behaviour. Behavioural data processing, thus, is expected to impact on policyholders (who know that their behaviour is monitored), on insurance companies (which can improve their predicting capacity by combining behavioural and non-behavioural variables), and on the relationship between policyholders and insurance companies (triggering feedback loops).

\green{What happens in practice? Is behavioural data-based motor insurance actually working, and how? The usual abstract assumption is that coaching works because policyholders who receive feedback improve their driving style and become better drivers  \cite[p.~22]{soleymanian2019sensor}. This assumption, yet, leaves open many questions which should be investigated more thoroughly. They concern, particularly, the interplay between feedback and improvement in driving behaviour, since the information fed back can be effective and produce a coaching effect only if the driver is engaged. In the next section, we briefly describe relevant research on the effectiveness of monitoring in motor insurance.}


==> Ref.tex <==


\section*{References}


\begin{hangparas}{2em}{1}
    Arrow, Kenneth (1971),   “Uncertainty and the Welfare Economics of Medical Care.” In \textit{Essays in the Theory of Risk-Bearing}, 177–211. Amsterdam and London: North-Holland.
  \end{hangparas}
\begin{hangparas}{2em}{1}
    Asimakopoulos, Stavros, Asimakopoulos, Grigorios \& Spillers, Frank (2017). “Motivation and User Engagement in Fitness Tracking: Heuristic for Mobile Healthcare Wearables.” \textit{Informatics}, 4(5), 1–16.
  \end{hangparas}
\begin{hangparas}{2em}{1}  
Baker, Tom \& Simon, Jonathan (2002). “Embracing Risk.” In Embracing Risk. The Changing Culture of Insurance and Responsibility, edited by Tom Baker and Jonathan Simon, 1–25. Chicago, \textit{IL and London: The University of Chicago Press.}
  \end{hangparas}
\begin{hangparas}{2em}{1}
Bolderdijk, Jan Willem, Knockaert, Jsa, Steg, Linda \& Verhoef, Erik T. (2011). “Effects of Pay-As-You-Drive Vehicle Insurance on Young Drivers’ Speed Choice: Results of a Dutch Field Experiment.” \textit{Accident Analysis and Prevention}, 43(3), 1181–1186.
  \end{hangparas}
\begin{hangparas}{2em}{1}  
Bucher, Amy (2020). “Engaged: Designing for Behavior Change.” \textit{New York: Rosenfeld Media}.
  \end{hangparas}
\begin{hangparas}{2em}{1} Cevolini, Alberto (2022). “ Coaching in Telematics Insurance: Control or Motivation?” Movingdots by Powerfleet. \url{https://www.movingdots.com/news-insights/coaching-strategies-in-telematics-motor-insurance-control-or-motivation} [last access May 18, 2023].
  \end{hangparas}
\begin{hangparas}{2em}{1} Cevolini, Alberto \& Esposito, Elena (2022). “From Actuarial to Behavioural Valuation: The Impact of Telematics on Motor Insurance.” \textit{Valuation Studies}, 9(1), 109–139.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Cultu, Deniz, Tamayo, Ganjani, Kristen, Larrea, Elixabete \& Müssig, Michael (2022). “Claims 2030: Dream or Reality?” McKinsey \& Company. \url{https://www.mckinsey.com/industries/financial-services/our-insights/claims-2030-dream-or-reality#/} [last access May 18, 2023].   
  \end{hangparas}
\begin{hangparas}{2em}{1} Discovery (2020). “ How the Vitality Drive Programme Works.” Discovery Insure. \url{https://www.discovery.co.za/assets/discoverycoza/car-and-home-insurance/vitality-drive-terms-and-conditions.pdf} [last access May 18, 2023]. 
  \end{hangparas}
\begin{hangparas}{2em}{1} Donaldson, Greg (2020). “Effective Driver Coaching Partnered With Telematics Improves Auto Claims and Customers Loyalty.” AITE Group Report prepared for Adept Driver. \url{ https://www.adeptdriver.com/assets/resources/Effective-Driver-Coaching-Partnered-With-Telematics-02-21-2020.pdf} [last access May 18, 2023].   
  \end{hangparas}

  
\begin{hangparas}{2em}{1} Ericson, Richard, Doyle, Aaron \& Barry, Dean (2003). “Insurance as Governance.” Toronto, ON: University of Toronto Press.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Farmer, Charles M., Kirley, Bevan B. \& McCartt, Anne T. (2010). “Effects of In-Vehicle Monitoring on the Driving Behaviour of Teenagers.” \textit{Journal of Safety Research}, 41(1), 39–45.    
  \end{hangparas}
\begin{hangparas}{2em}{1} Gorm, Nanna \& Shklovski, Irina (2019). “Episodic Use: Practices of Care in Self-Tracking.” \textit{New Media \& Society}, 21(11-12), 2505–2521.    
  \end{hangparas}
\begin{hangparas}{2em}{1} Guillen, Montserrat, Nielsen, Jens Perch, Ayuso, Mercedes \& Pérez-Marín, Ana M. (2019). “ The Use of Telematics Devices to Improve Automobile Insurance Rates.” \textit{Risk Analysis}, 39(3), 662–672. 
  \end{hangparas}
\begin{hangparas}{2em}{1} Guillen, Montserrat \& Cevolini, Alberto (2021). “Using Risk Analytics to Prevent Accidents Before They Occur – The Future of Insurance.” \textit{Journal of Financial Transformation}, 54, 76–83.   
  \end{hangparas}
\begin{hangparas}{2em}{1} Händel,  Peter, Skog, Isaac \& Wahlström, Johan (2014). “Insurance Telematics: Opportunities and Challenges With the Smartphone Solution.” \textit{IEEE Intelligent Transportation Systems Magazine}, 6(4), 57–70.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Heimer, Carol (1985). “Reactive Risk and Rational Action. Managing Moral Hazard in Insurance Contracts.” Berkeley, CA: University of California Press.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Lasry, Jean-Michel (2015). “La rencontre choc de l’assurance et du Big Data.” \textit{Risques}, 103, 19–24.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Litman, Todd (2005). “Pay-As-You-Drive Pricing and Insurance Regulatory Objectives.” \textit{Journal of Insurance Regulation}, 23(3), 35–53.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Lupton, Deborah (2013). “The Digitally Engaged Patient. Self-Monitoring and Self-Care in the Digital Health Era.” \textit{Social Theory \& Health}, 11(3), 256–270.     
  \end{hangparas}
  
\begin{hangparas}{2em}{1} Lupton, Deborah (2016). “The Diverse Domains of Quantified Selves: Self-Tracking Modes and Dataveillance.” \textit{Economy \& Society}, 45(1), 101–122.    
  \end{hangparas}
\begin{hangparas}{2em}{1} Meyers, Gert \& Van Hoyweghen, Ine (2017). “Enacting Actuarial Fairness in Insurance: From Fair Discrimination to Behaviour-Based Fairness.” \textit{ Science as Culture}, 27(4), 413–438. 
  \end{hangparas}
\begin{hangparas}{2em}{1} Picard, Florence (2018). “Current Vision and Market Prospective.” \textit{Big Data for Insurance Companies}, edited by Marine Corlosquet-Habart \& Jacques Janssen, 83–129. London: John Wiley \& Sons.
  \end{hangparas}
\begin{hangparas}{2em}{1} Romanelli, Lorenzo \& Albers, Sandra (2021).  “Are You the Best Driver on the Road?” Movingdots by Powerfleet. \url{https://www.movingdots.com/news-insights/are-you-the-best-driver-on-the-road} [last access May 18, 2023]. 
  \end{hangparas}
\begin{hangparas}{2em}{1} Ruckenstein, Minna \& Pantzar, Mika (2017). “Beyond the Quantified Self: Thematic Exploration of a Dataistic Paradigm.” \textit{New Media}, 19(3), 401–418.    
  \end{hangparas}
\begin{hangparas}{2em}{1} Siegelman, Peter (2014). “Information and Equilibrium in Insurance Markets With Big Data.” \textit{Connecticut Insurance Law Journal}, 21(1), 317–338.    
  \end{hangparas}
\begin{hangparas}{2em}{1} Soleymanian, Miremad, Weinberg, Charles B. \& Zhu, Ting (2019). “Sensor Data and Behavioural Tracking: Does Usage-Based Auto Insurance Benefit Drivers?” \textit{Marketing Science}, 38(1), 21–43.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Stevenson, Mark, Harris, Anthony, Wijnands, Jasper S. \& Mortimer, Duncan (2021). “The Effects of Telematics Based Feedback and Financial Incentives on Driving Behaviour: A Randomised Trial.” \textit{Accident Analysis and Prevention}, 159, 1–8.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Stiglitz, Joseph (1983). “Incentives and Insurance: The Pure Theory of Moral Hazard.” \textit{The Geneva Papers on Risk and Insurance}, 8(26), 4–33.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Stone, Deborah (2002). “Beyond Moral Hazard: Insurance as Moral Opportunity”. \textit{Embracing Risk. The Changing Culture of Insurance and Responsibility}, edited by Tom Baker \& Jonathan Simon, 52–79. Chicago, IL and London: The University of Chicago Press. 
  \end{hangparas}
  
  
\begin{hangparas}{2em}{1} Tanninen, Maiju, Lehtonen, Turo-Kimmo \& Ruckenstein, Minna (2021). “Tracking Lives, Forging Markets.” \textit{Journal of Cultural Economy}, 14(4), 449–463.    
  \end{hangparas}
\begin{hangparas}{2em}{1} Tanninen, Maiju, Lehtonen, Turo-Kimmo \& Ruckenstein, Minna (2022).  “The Uncertain Element. Personal Data in Behavioural Insurance.” \textit{Climate, Society and Elemental Insurance. Capacities and Limitations}, edited by Kate Booth, Chloe Lucas \& Shaun French, 187–200. London and New York: Routledge. 
  \end{hangparas}
\begin{hangparas}{2em}{1} Wahlström, Johan, Skog, Isaac \& Händel, Peter (2015). “Driving Behaviour Analysis for Smartphone-Based Insurance Telematics.” \textit{Proceedings of the 2nd Workshop on Physical Analytics - WPA ’15}, 19–24.  
  \end{hangparas}
\begin{hangparas}{2em}{1} Weidner, Wiltrud, Transchel, Fabian W. G.  \& Weidner, Robert (2017). “ Telematic Driving Profile Classification in Car Insurance Pricing.” \textit{Annuals of Actuarial Science}, 11(2), 213–236. 
  \end{hangparas}
\begin{hangparas}{2em}{1} Wouters, Peter \& Bos, John (2000). “Traffic Accident Reduction by Monitoring Driver Behaviour With In-Car Data Recorders.” \textit{Accident Analysis \& Prevention}, 32(5), 643–650.    
  \end{hangparas}
\begin{hangparas}{2em}{1} Ziakopoulos, Apostolos, Petraki, Virginia, Kontaxi, Armira \& Yannis, George (2022). “The Transformation of the Insurance Industry and Road Safety by Driver Safety Behaviour Telematics.” \textit{Case Studies on Transport Policy}, 10(4), 2271–2279.    
  \end{hangparas}

